Quasi-coherent sheaves on the moduli stack of formal groups

The central aim of this monograph is to provide decomposition results for quasi-coherent sheaves on the moduli stack of one-dimensional formal groups. These results will be based on the geometry of the stack itself, particularly the height filtration and an analysis of the formal neighborhoods of the geometric points. The main theorems are algebraic chromatic convergence results and fracture square decompositions. There is a major technical hurdle in this story, as the moduli stack of formal groups does not have the finitness properties required of an algebraic stack as usually defined. This is not a conceptual problem, but in order to be clear on this point and to write down a self-contained narrative, I have included a great deal of discussion of the geometry of the stack itself, giving various equivalent descriptions.

==> formalgrps.tex <==
\section{Formal Groups}

This section is devoted to a rapid introduction to schemes,
formal schemes, and -- most importantly --
smoothness for formal schemes.
This is so we can have a definition of formal group which 
does not depend {\it a priori} on a theory of coordinates.

\subsection{Schemes as functors: a brief introduction}

Let $R$ be a commutative ring and let
$\Alg_R$ be the category of R-algebras; this category is
equivalent to the
opposite category of the category of affine schemes over $\Spec(R)$.
Schemes over $R$ can be thought of as functors from $\Alg_R$
to the category of sets. We briefly review this material,
mostly to establish language. 

The basic schemes over $R$ are the affine schemes $\Spec(B)$,
where $B$ is an $R$-algebra. As a functor
$$
\Spec(B):\Alg_R \longr \Sets
$$
is the representable functor determined by $R$; that is,
$$
\Spec(B)(A) = \Alg_B(B,A).
$$
If $I \subseteq B$ is an ideal
we have the open subfunctor $U_I \subseteq \Spec(B)$ with
$$
U_I(A) =\{\ f:B \to A\ |\ f(I)A = A\ \} \subseteq \Spec(B).
$$
This defines the Zariski topology on $\Spec(B)$.
The complement of $U_I$ is the closed subfunctor $Z_I = \Spec(B/I)$.
Note that we can guarantee that
$$
U_I(A) \cup Z_I(A) = \Spec(B)(A)
$$
only if $A$ is a field.

If $X: \Alg_R \to \Sets$ is any functor, we define a subfunctor 
$U \subseteq X$ to be {\it open} if the subfunctor
$$
U \times_X \Spec(B) \subseteq \Spec(B)
$$
is open for for all morphisms of functors $\Spec(B) \to X$. Such morphisms
are in one-to-one correspondence with $X(B)$, by the Yoneda Lemma.
A collection of subfunctors $U_i \subseteq X$ is called a cover
if the morphism $\sqcup U_i(\FF) \to X(\FF)$ is onto for all
{\it fields} $\FF$.

As a matter of language, a functor $X:\Alg_R \to \Sets$ will be called an
{\it $R$-functor}.

\begin{defn}\label{scheme}An $R$-functor $X$ is a {\it scheme over
$R$} if 
it satisfies the following two conditions:
\begin{enumerate}

\item $X$ is a sheaf in the Zariski topology; that is, if $A$ is
an $R$-algebra and $a_1,\ldots,a_n \in A$ are elements so that
$a_1 + \cdots + a_n = 1$, then
$$
\xymatrix{
X(A) \rto & \prod X(A[a_i^{-1}]) \ar@<.5ex>[r] \ar@<-.5ex>[r] &
\prod X(A[a_i^{-1}a_j^{-1}])
}
$$
is an equalizer diagram; and

\item $X$ has an open cover by affine schemes $\Spec(B)$ where
each $B$ is an $R$-algebra

\end{enumerate}
A morphism $X \to Y$ of schemes over $R$ is a natural transformation
of $R$-functors.
\end{defn}

The basic example of a scheme which is not affine is projective
space $\PP^n$ which assigns to each ring $A$ the set of
direct factors of rank $1$ of $A^{n+1}$.

If $X$ is any $R$-functor, define $\Aff/X$ to the category with
objects the morphisms of $R$-functors $\Spec(B) \to X$;
morphisms are commutative triangles. We give this category
the {\it fpqc}-topology\footnote{The acronym $fpqc$ stands for ``fid\`element
plat quasi-compact''. It is not yet a topology as the category is
not closed under base change. See Remark \ref{fpqc} below.}
as follows: $\Spec(B') \to \Spec(B) \to X$ will
be open if $\Spec(B') \to \Spec(B)$ is flat. An open
cover will be finite collection of flat morphisms $\Spec(B_i) \to \Spec(B)$
so that $\sqcup \Spec(B_i) \to \Spec(B)$ is surjective. It is
equivalent to say that $B \to \prod B_i$ is faithfully flat; thus,
it is sufficient to consider covers by a single morphism.

\begin{defn}\label{O-X}Let $X$ be an $R$-functor. We
define three basic types of sheaves on $\Aff/X$.
\begin{enumerate}

\item The {\bf structure sheaf} $\cO_X = \cO$ of $X$ is the functor
$$
\cO_X:(\Aff/X)^{op} \longr \Alg_R
$$
given by $\cO_X(\Spec(B) \to X) = B$. This is a sheaf in the
$fpqc$ topology.

\item An {\it $\cO_X$-module sheaf} is a functor
$$
\cF: (\Aff/X)^{op} \longr \Sets
$$
so that $\cF$ is a sheaf in the $fpqc$-topology and so that
$\cF(\Spec(B) \to X)$  is naturally a $B$-module. Write
$\Mod_X$ for the category of $\cO_X$-module sheaves.

\item An $\cO_X$-module sheaf $\cF$ is {\it quasi-coherent} if
for all morphisms $\Spec(B') \to \Spec(B) \to X$ over $X$,
the induced map
\begin{equation}\label{tensor-up}
B' \otimes_B \cF(\Spec(B) \to X) \to \cF(\Spec(B') \to X)
\end{equation}
is an isomorphism. Write $\Qmod_X$ for the category
of quasi-coherent sheaves over $X$. 
\end{enumerate}
\end{defn}

To simplify notation, we may write
$\cF(B)$ or $\cF(\Spec(B))$ for $\cF(\Spec(B) \to X)$.

\begin{rem}\label{qc-sheaf-rems} 1.) If $\cF$ is an
$\cO_X$-module sheaf over an $R$-functor $X$, the
{\it global sections} of $\cF$ are given by 
$$
\Gamma(X,\cF) = H^0(X,\cF) = \lim_{\Aff/X}\cF(\Spec(A) \to X).
$$
The cohomology groups $H^n(X,\cF)$ are the right derived functors
of global sections; these are the cohomology groups of the cochain complex
$R\Gamma(X,\cF)$ -- the total
right derived functor of $\Ga(X,-)$ applied to $\cF$. This is
well defined object in the homotopy category of cochain complexes
of $\cO_X$-modules sheaves. This homotopy category is
the {\it derived category} of module sheaves.

2.) If $X = \Spec(S)$ for some $R$-algebra $S$ and $M$ is a 
$S$-module, get quasi-coherent sheaf $\tilde{M}$ on
$X$ with
$$
\tilde{M}(\Spec(B) \to X) = B \otimes_S M.
$$
We have immediately that 
$H^0(\Spec(B),\tilde{M})=M$; thus, there is
an equivalence of categories between $S$-modules
and quasi-coherent sheaves on $\Spec(S)$.

3.) Note that any presheaf $\cF$ of $\cO_X$-modules
which satisfies Equation \ref{tensor-up} is automatically a sheaf, by
faithfully flat descent. 

4.) An important example of an $\cO_X$ module
sheaf which is not quasi-coherent for the flat topology is the 
cotangent sheaf $\Omega_{X/R}$ with
$$
\Omega_{X/R}(\Spec(B) \to X) = \Omega_{B/R}.
$$

5.) If $f:X \to Y$ is a morphism of $R$-functors and $\cF$ is
an $\cO_Y$-module sheaf, define $f^\ast \cF$ to be the $\cO_X$-module
sheaf with 
$$
f^\ast \cF(\Spec(B) \to X) = \cF(\Spec(B) \to X \to Y).
$$
This is a quasi-coherent sheaf if $\cF$ is quasi-coherent. As examples,
$f^\ast \cO_Y \cong \cO_X$, but the natural map $f^\ast \Omega_{Y/R} \to
\Omega_{X/R}$ is often not an isomorphism. Also, if
$f:\Spec(B') \to \Spec(B)$ is a morphism
of affine schemes and $M$ is a $B$-module, then
$$
f^\ast \tilde{M} = \widetilde{B' \otimes_B M}.
$$
We will discuss the right adjoint $f_\ast$ of $f_\ast$ below
in Definition \ref{push-forward} and Proposition \ref{push-forward-qc}.

6.)  If $\cF$ is an $\cO_X$-module sheaf over an $R$-functor $X$, then
$U$ extends uniquely to a functor on the category of all schemes
$U$ over $X$ by setting
$$
\cF(f:U \to X) = H^0(U,f^\ast \cF).
$$
Note that $\cO_X(U) = H^0(U,\cO_U)$.

7.) There is an evident notion of an $\cO_X$-algebra sheaf and of
a quasi-coherent $\cO_X$-algebra sheaf. If $\cA$ is $\cO_X$-algebra
sheaf, there is also an evident notion of a $\cA$-module sheaf and
of a quasi-coherent $\cA$-module sheaf. And $\cA$-module sheaf
is an $\cO_X$-module sheaf by restriction of scalars.
\end{rem}

To say much more, we have to introduce some constructions and hypotheses.
A morphism $X \to Y$ of $R$-functors is called {\it schematic} if
for all morphisms $U \to Y$ with $U$ a scheme, the pull-back
$U \times_Y X$ is scheme. Any morphism of schemes is automatically
schematic. 

\begin{defn}\label{push-forward}Let $f:X \to Y$ be a schematic
morphism of $R$-functors and let $\cF$ be an $\cO_X$-module 
over $X$. Then the push-forward $f_\ast \cF$ of $\cF$ is defined by
$$
(U \to Y) \mapsto \cF(U \times_Y X \to X) = H^0(U \times_Y X,\cF).
$$
There is a natural map of sheaves $\cO_Y \to f_\ast \cO_X$; in fact,
$f_\ast \cO_X$ is a $\cO_Y$-algebra sheaf and $f_\ast \cF$ is
then becomes an $\cO_Y$-module sheaf.
\end{defn}

The functor $f_\ast:\Mod_X \to \Mod_Y$ is right adjoint to the
functor $f^\ast$. By it's very definition it's clear that the
push-forward is not exact. Let $Rf_\ast \cF$ be the total
right derived functor of the push-forward. There are hypotheses
that we guarantee that $f_\ast$ is exact; for example,
if $f:\Spec(B') \to \Spec(B)$ and $M$ is $B'$ module, then
$f_\ast\tilde{M} = \tilde{M}$, where $M$ is a $B$-module
by restriction of scalars. See also Proposition \ref{qc-affine}.

If $P$ is any property of morphisms of schemes which is
stable under pull-back, then $P$ can be extended to schematic
morphisms $f:X \to Y$ of $R$-functors by saying that $f$
has property $P$ if and only if $U \times_Y X\to U$ has
property $P$ for all morphism $U \to Y$ with $U$ a
scheme. We implicitly used this concept already when defining
the notion of an open sub-functor; here we spell it out in more
detail in the following examples. 

\begin{defn}\label{cool-morphisms-1}1.) Let $f:X \to Y$ be a 
schematic morphism of $R$-functors. Them $f$ is {\bf flat}
if for all morphisms $U \to Y$ where $U$ is a scheme, the
morphism of rings $\cO_Y(U) \to f_\ast\cO_X(U)$ is flat.
Also $f$ is faithfully flat if it flat and surjective.

2.) Let $f:X \to Y$ be a morphism of schemes. Then $f$ is
{\bf locally of finite-type} if $Y$ has a cover by open
subschemes $U \to Y$ so that
$$
\cO_Y(U) \to f_\ast\cO_X(U)
$$
presents $f_\ast\cO_X(U)$ as a finitely generated $\cO_Y(U)$
algebra.
\end{defn}

\begin{rem}[Faithfully flat descent]\label{ff-descent}Let $f:X \to Y$ be an morphism
if $R$-functors. Let 
$$
X^n = X \times_Y \cdots \times_Y X
$$
where the product is taken $n$-times and let $\phi:[m] \to [n]$ be any morphism
in the ordinal number category. Define $\phi^\ast :X^n \to X^m$ be the formula
$$
\phi(x_0,\ldots,x_n) = (x_{\phi(0)},\cdots,x_{\phi(n)}).
$$
In this way we obtain a simplicial $R$-functor $X_\bullet$ augmented to $Y$.
This is the {\it coskeleton} of $f$. 

A {\it descent problem} for $f$ is a pair $(\cF,\psi)$ where $\cF$ is a sheaf on
$X$ and $\psi:d_1^\ast \cF \to d_0^1 \cF$ is an isomorphism of sheaves
on $X \times_Y X$ subject to the cocycle condition
$$
d_1^\ast \psi = d_2^\ast \psi d_0^\ast \psi
$$
over $X \times_Y X \times_Y X$. A solution to a descent problem is a sheaf
$\cE$ over $Y$ an isomorphism $\phi_0:f^\ast \cE \to \cF$ over $X$
so that the following diagram commutes
$$
\xymatrix{
d_1^\ast f^\ast \cE \rto^{c} \dto_{d_1^\ast \psi_0}
& d_0^\ast f^\ast \cE \dto^{d_0^\ast \psi_0}\\
d_1^\ast \cF \rto_{\psi} & d_0^\ast \cF
}
$$
where $c$ is the canonical isomorphism obtained from the equation $fd_1 = fd_0$.
If $f:X \to Y$ is flat and $(\cF,\psi)$ is a descent problem with $\cF$ quasi-coherent,
then there is at most one solution with $\cE$ quasi-coherent. If $f$ is faithfully
flat, there is exactly one solution and we get an evident equivalence of categories.
This has many refinements; for example, one could concentrate on algebra sheaves
instead of module sheaves.
\end{rem}

The push-forward functor does not always preserve quasi-coherent
sheaves, so we make the following definitions as well.

\begin{defn}\label{cool-morphisms-2}
1.) A scheme $X$ is called {\bf quasi-compact} if every cover by open
subschemes $U_i \subseteq X$ has a finite subcover. A morphism of
schemes $X \to Y$ is quasi-compact if for every quasi-compact
open $V \subseteq Y$, the scheme $V \times_Y X$ is quasi-compact.
This notion then extends to schematic morphisms of $R$-functors.

2.) A morphism $f:X\to Y$ of $R$-functors is called
{\bf quasi-separated} if the diagonal morphism 
$X \to X \times_Y X$ is schematic and quasi-compact.
An $R$-functor $X$ is quasi-separated if the unique morphism
$X \to \Spec(R)$ is quasi-separated.
\end{defn}

The following is in \cite{DG}, Proposition I.2.2.4.

\begin{prop}\label{push-forward-qc}Let $f:X \to Y$ be
a quasi-compact and quasi-separated morphism of schemes.
If $\cF$ is a quasi-coherent $\cO_X$-module sheaf, then
$f_\ast \cF$ is a quasi-coherent $\cO_Y$ module sheaf,
and $f_\ast:\Qmod_X \to \Qmod_Y$ is right adjoint to
$f^\ast$.
\end{prop}

\begin{rem}[The $fpqc$-topology and the Zariski topology]\label{fpqc}Let $X$ be
an $R$-functor and suppose that the diagonal map
$X \to X \times_{\Spec(R)} X$ is schematic. Then any morphism
$V \to X$ with $V$ a scheme is schematic. Define the $fpqc$-topology
on $X$ as follows. The basic opens are the quasi-compact
morphisms $V \to X$ with $V$ a scheme. A cover of $V \to X$ is a finite
set of flat and quasi-compact morphisms $V \to R$ 
so that $\coprod V_i \to V$ is surjective. 

There are times when we will need the {\it Zariski topology}
as well. In this case a basic open is an open inclusion
$V \to X$ where $V$ is as scheme; a cover of $V$ is
a set of open inclusions $V_i \to V$ so that $\sqcup V_i \to V$
is surjective. 
\end{rem}

Let $\Mod_X^{Zar}$ and
$\Mod_X^{fqqc}$ be the categories of $\cO_X$-module
sheaves in the Zariski  and $fpqc$-topologies respectively.
If $I$ is a set, write $\cO_X^{(I)}$ for $\coprod_I \cO_X$
in either category. 

Recall that $\cF \in \Mod_X^{Zar}$ is said to be quasi-coherent
if there is an open cover by open subschemes $V \subseteq X$
so that for each $V$ there are sets $I$ and $J$ and
exact sequence of sheaves
$$
\cO_V^{(J)} \longr \cO_V^{(I)} \to \cF\vert_V
$$
We reconcile this notion of quasi-coherent with that given
in Definition \ref{O-X}.

Let $X$ be a quasi-compact and quasi-separated scheme.
Then every open morphism $U \to X$ is flat and 
quasi-compact; hence, there is a restriction morphism
$$
\epsilon_\ast:\Mod_X^{fpqc} \longr \Mod_X^{Zar}.
$$
The functor $\epsilon_\ast$ has a left adjoint $\epsilon^\ast$: if
$\cF \in \Mod_X^{Zar}$ then for each flat and
quasi-compact morphism $f:U \to X$ we have a $\cO_U$-module
sheaf $f^\ast \cF$ and these assemble into a presheaf. 
If $\cF$ is quasi-coherent as a sheaf in the Zariski topology, this is already
a sheaf, by faithfully flat descent. In the more general case, let
$\epsilon^\ast\cF$ be the associated sheaf. 

\begin{defn}\label{cartesian} Let $\cF \in \Mod_X^{fpqc}$ an
an $\cO_X$-module sheaf in the $fpqc$-topology. Then $\cF$
is {\it cartesian} if for any diagram
$$
\xymatrix@R=5pt{
V \ar[dd]_f \ar[dr]^y\\
& X\\
U \ar[ur]_x
}
$$
with all three of $f$, $x$, and $y$ flat and quasi-compact, the 
natural map in $\Mod_V^{Zar}$
$$
f^\ast \cF_U \longr \cF_V
$$
is an isomorphism.
\end{defn}

The following is clear.

\begin{lem}\label{epsilon-is-cart} Let $\cN \in \Mod_X^{Zar}$ be a
quasi-coherent sheaf on $X$. Then $\epsilon^\ast \cN
\in \Mod_X^{fpqc}$ is cartesian and for each flat and quasi-compact
morphism $f:U \to X$, the $\cO_U$-module sheaf $f^\ast \cN$
is quasi-coherent as a sheaf in the Zariski topology.
\end{lem}

\begin{prop}\label{conditions-for-qc} Let $X$ be a be a quasi-compact
and quasi-separated scheme and
$\cF$  a sheaf of  $\cO_X$ modules in the $fpqc$-topology. Then the following conditions are equivalent.
\begin{enumerate}

\item The sheaf $\cF$ is cartesian and for each flat and
quasi-compact morphism $U \to X$ the $\cO_U$-module
sheaf $\cF_U$ is quasi-coherent in the Zariski topology.

\item The sheaf $\epsilon_\ast \cF = \cF_X$ is quasi-coherent and the
induced morphism $\epsilon^\ast\epsilon_\ast \cF \to \cF$
is an isomorphism.

\item There is a flat surjective quasi-compact morphism $p:Y \to X$
and sets $I$ and $J$ so that there is an exact sequence of
sheaves in $\Mod_Y^{fpqc}$
$$
\xymatrix{
\cO_Y^{(J)} \rto & \cO_Y^{(I)} \rto & p^\ast\cF \rto &0.
}
$$
\end{enumerate}
\end{prop}

\begin{proof} $(1) \Rightarrow (2)$: We are assuming $\epsilon_\ast\cF$
is quasi-coherent. Now let $f:U \to X$ be flat and quasi-compact. Then
$$
(\epsilon^\ast\epsilon_\ast\cF)_U = f^\ast\cF_X \cong \cF_U.
$$

For $(2) \Rightarrow (1)$ use Lemma \ref{epsilon-is-cart}.

For $(1) \Rightarrow (3)$ take $Y = \sqcup U_i$ where $\{ U_i \to X\}$
is a finite cover by affine Zariski opens.

For $(3) \Rightarrow (1)$ use faithfully flat descent: $p^\ast \cF$
is cartesian and locally quasi-coherent in the Zariski topology.
Now check that both of these properties descend.
\end{proof}

Define $\Cart_X$ to be the full-subcategory
of $\Mod_X^{fpqc}$ with objects the module sheaves $\cF$ which
satisfy the three equivalent conditions of Proposition \ref{conditions-for-qc}.
An immediate consequence of  Proposition \ref{conditions-for-qc}.2
is the next result:

\begin{prop}\label{qc-indep-topology} Let $X$
be a quasi-compact and quasi-separated scheme. The adjoint functors
$$
\xymatrix{
\epsilon^\ast: \Mod_X^{Zar} \ar@<.5ex>[r] & \ar@<.5ex>[l]
\Mod_X^{fpqc}:\epsilon_\ast
}
$$
restrict to an equivalence of categories between quasi-coherent
sheaves in the Zariski topology and $\Cart_X$.
\end{prop}

Let $\Mod_X$ be the category of $\cO_X$-module sheaves
as defined in Definition \ref{O-X}. The following is in
\cite{DG} \S I.2.4.5.

\begin{prop}\label{qc-indep-topology-2}There are adjoint functors
$$
\xymatrix{
\eta^\ast:\Mod_X^{Zar} \ar@<.5ex>[r] &  \ar@<.5ex>[l]:\Mod_X:\eta_\ast
}
$$
which restrict an equivalence of categories between $\Qmod_X$
and and the quasi-coherent sheaves on $X$ in the Zariski topology.
\end{prop}

The functor $\eta_\ast$, for example, assigns to each $\cO_X$-module
sheaf $\cF$ the sheaf $\eta_\ast\cF$ in the Zariski topology 
associated to the presheaf
$$
U \longmapsto H^0(U,\cF\vert_U).
$$

As a result of Propositions \ref{qc-indep-topology} and Proposition
\ref{qc-indep-topology-2}, we will refer to the sheaves in all of these
categories as quasi-coherent sheaves. A quasi-coherent sheaf
will be {\it coherent} is it locally finitely presented; that is,
the sets $I$ and $J$ of Proposition \ref{conditions-for-qc}.3
can be chosen to be finite.

\begin{lem}\label{fflat-inherits}Let $f:Y \to X$ be a faithfully
flat and quasi-compact morphism of schemes and suppose $X$
is quasi-compact and quasi-separated. Then the following
properties of quasi-coherent sheaves descend. Let
$\cF \in \Qmod_X$.
\begin{enumerate}

\item The quasi-coherent sheaf $M$ is flat if and only if $f^\ast \cF$ is flat.

\item The quasi-coherent sheaf $M$ is coherent
if and only if $f^\ast\cF$ is coherent.

\item Suppose that $\cF$ is coherent. Then $\cF$ is locally free
if and only $f^\ast \cF$ is locally free. It is locally of rank $n$
if and only if $f^\ast \cF$ is locally free of rank $n$.

\item Let $X' \to X$ be any morphism. Then $Y \times_X X' \to X'$
is faithfully flat and quasi-compact.
\end{enumerate}
\end{lem}

\begin{proof}These are all in \cite{EGAIV}\S 2.6.
\end{proof}

We finish this section with a review of an important class of morphisms.

\begin{defn}\label{affine-morphisms}1.) A morphism $f:X \to Y$
of $R$-functors is called {\bf affine} if for all morphisms
$\Spec(B) \to Y$, the $R$-functor $\Spec(B) \times_Y X$
is isomorphic to an affine scheme. 

2.) A morphism $f:X \to Y$ of $R$-functors 
is a {\bf closed embedding} if it is affine and for all morphisms
$\Spec(B) \to Y$, the induced morphisms of rings
$$
B = \cO_Y(B) \longr f_\ast \cO_X(B) = \cO_X(\Spec(B) \times_Y X 
\to X)
$$
is surjective.

3.) A morphism $f:X \to Y$ of schemes over $R$ is {\bf separated} if the
diagonal morphism $X \to X \times_Y X$ is a closed embedding.
\end{defn}

If $f:X \to Y$ is an affine morphism of schemes, then the $\cO_Y$ algebra
sheaf $f_\ast \cO_X$ is quasi-coherent. Conversely, if
$\cB$ is quasi-coherent $\cO_Y$-algebra sheaf, define
a $R$-functor $\Spec_Y(\cB)$ over $Y$ by
$$
\Spec_Y(\cB)(A) = \coprod_{\Spec(A) \to Y} \Alg_A(\cB(\Spec(A) \to Y),A).
$$
Then $q:\Spec_Y(\cB) \to Y$ is an affine morphism of $R$-functors
and $q_\ast \cO_{\Spec_Y(\cB)} \cong \cB$. This gives an equivalence
between the category of quasi-coherent $\cO_Y$-algebras and
the category of affine morphisms over $Y$.

An analogous result holds for quasi-coherent sheaves.

\begin{prop}\label{qc-affine}Let $f:X \to Y$ be an affine morphism
of schemes. Then the push-forward functor $f_\ast$ defines
an equivalence of categories between quasi-coherent
sheaves on $X$ and quasi-coherent $f_\ast \cO_X$-module
sheaves on $Y$. In particular, $f_\ast$ is exact.
\end{prop}

\begin{proof}First, it follows immediately from the definition
of an affine morphism that $f_\ast$ takes quasi-coherent
sheaves to quasi-coherent sheaves; from this it we deduce
that $f_\ast \cF$ is quasi-coherent sheaf of
$f_\ast \cO_X$-modules. We next define the functor back.

From the correspondence of the previous paragraph, we
see that to specify a morphism $i:\Spec(A) \to X$ it is
sufficient to specify the pair $(fi,\phi)$ where
$fi:\Spec(A) \to Y$ is the composition and 
$$
\phi:f_\ast \cO_X(fi:\Spec(A) \to Y) \to A
$$
is an $A$-algebra homomorphism. If $\cE$ is a quasi-coherent
$f_\ast \cO_X$-module sheaf, define a quasi-coherent sheaf $\cF$
on $X$ by
$$
\cF(i:\Spec(A) \to X) = A \otimes_\phi \cE(fi:\Spec(A) \to Y).
$$
Here $\otimes_\phi$ means tensor over $f_\ast \cO_X(fi:\Spec(A) \to Y)$
where $A$ becomes a module over this ring via $\phi$.

We easily check these two functors are inverses of each other.
\end{proof}

\subsection{Formal schemes}

The notion of formal scheme was defined and discussed in \cite{EGA} \S 10.
We will be interested in a specialization of the general case where we,
in effect, make the ``ideal of definition'' of the formal scheme part
of the data.

Specifically, we will have a scheme $S$ and
a morphism of $R$-functors $q:X \to S$
with a section $s:S \to X$; that is, $qs = 1:S \to S$. The $R$-functor
$X$ will be a formal scheme and the inclusion $s:S \to X$ will
indentify $S$ with the scheme defined by a fixed ideal of
definition of $X$.  We now explain what all this means.

\begin{defn}\label{formal-scheme}Let $S$ be a scheme 
over a commutive ring $R$ and let $S \to X$ be a
closed embedding of $R$-functors defined by an ideal
$\cI \subseteq \cO_X$. Let $X_n \subseteq X$
be the closed embedding defined by $\cI^n$. The
inclusion $S \to X$ is {\bf formal} if each
$X_n$ is a scheme over $R$ and 
$$
X = \colim_n X_n.
$$
\end{defn}

\begin{exam}\label{frml-nghbd}1.) If $(B,I)$ be an $R$-algebra
with an ideal $I$. Then
$$
\Spf(B) \defeq \{\ f:B \to A\ |\ f(I)A\ \hbox{is nilpotent}\ \}
= \colim_n \Spec(B/I^n)
$$
and the pair $\Spec(B/I) \to \Spf(B)$ is formal. The functor
$\Spf(B)$ depends only on the $I$-adic completion 
$B^\cmpl_I = \lim_n B/I^n$; thus, we usually assume that
$B$ is $I$-adically complete. The most basic example of this situation is
$\hat{\AA}^n_S = \Spf(R[[x_1,\ldots,x_n]])$, where
$R[[x_1,\ldots,x_n]]$ is the power series ring on $n$-variables
$I = (x_1,\cdots,x_n)$ is the maximal ideal.

2.) More generally, let $S \subseteq X$ be a closed embedding
of schemes  and let $\cI \subseteq \cO_X$ be the ideal
defining this embedding. Define
$$
X^\cmpl_S = \colim_n \Spec_X(\cO/\cI^n).
$$
Then the pair $S \to X_S^\cmpl$ is formal; this is the
{\it formal neighborhood} of $S$ in $X$.
\end{exam}

Let $S \to X$ be formal; write $i_n:X_n \to X$ for the
resulting family of closed inclusions. The following
results says that sheaves on $X$ are determined by
the pull-backs to the sheaves on $X_n$.

\begin{lem}\label{mod-formal}Let $S \to X$ be formal,
and let $\cF$ be an
$\cO_X$-module sheaf. Then the
natural morphism to the inverse limit
$$
\cF \longr \lim (i_n)_\ast i_n^\ast \cF = \lim \cF/\cI^n\cF
$$
is an isomorphism.
\end{lem}

\begin{proof}Let $\Spec(A) \to X$ be any morphism over $R$;
then, $\cI(A)^n = 0$ for some $n$. From this it follows
that
$$
\cF(A) \longr \cF(A)/\cI^n(A)\cF(A)
$$
is an isomorphism.
\end{proof}

\begin{exam}\label{qc-spf}In Remark \ref{qc-sheaf-rems}.2, we
recalled the equivalence between $B$-modules and quasi-coherent
sheaves over $\Spec(B)$. While analogous functors exist in the
formal setting, they do not give an equivalence in such generality.

Let $(B,I)$ be an $R$-algebra
with ideal $I$ and let $M$ be an $R$-module. Then,
using Example \ref{qc-sheaf-rems}.3, $M$
determines a quasi-coherent sheaf on $\Spec(B)$, hence,
by restriction, a quasi-coherent sheaf $M^\Delta$ on $X = \Spf(B)$. 
Then 
$$
(i_n)_\ast i_n^\ast M^\Delta = \widetilde{M/I^n M} = (M/I^nM)^\Delta.
$$
Note that $M^\Delta$ depends only on the $I$-adic completion
$M^\cmpl_I$ of $M$ and
$$
H^0(\Spf(B),M^\Delta) = \lim_{\Aff/\Spf(B)} \cF \cong M^\cmpl_I.
$$
If $\cF$ is a quasi-coherent sheaf on $\Spf(B)$, then
$$
H^0(\Spf(B), \cF) \cong \lim M_n \defeq M(\cF)
$$
is an $I$-adically complete $B$-module; however, the natural map
$\cM(\cF)^\Delta \to \cF$ is not always an isomorphism.
Thus we have an adjoint pair of functors between $I$-adically
complete $B$-module and quasi-coherent sheaves on $\Spf(B)$.
If $B$ is $I$-adically complete and Noetherian, this restricts to an
equivalence between the finitely generated $B$-modules and the
coherent sheaves on $\Spf(B)$. See \cite{EGA} \S 10.10.
\end{exam}

We now specialize the notion of a formal scheme.
Fix a scheme $S$ over a commutative
ring $R$. The we will consider the category of diagrams
$$
\xymatrix{
X \ar@<.5ex>[r]^-q & \ar@<.5ex>[l]^-s S
}
$$
where $q$ and $s$ are morphisms of $R$-functors, $s$ is
a section of $q$ and the pair $s:S \to X$ is formal. We will
call such diagrams {\it formal schemes augmented over $S$}.
If $B$ is $I$-adically complete and $B$ is a $B/I$ algebra, then
$$
\xymatrix{
\Spf(B) \ar@<.5ex>[r]^-q & \ar@<.5ex>[l]^-s \Spec(B/I)
}
$$
is an example.

\begin{lem}\label{formal-prod}The category of formal schemes
augmented over $S$ has finite products.
\end{lem}

\begin{proof} If $X$ and $Y$ are formal schemes augmented
over $S$, then the formal neighborhood of
$$
S \cong S \times_S S\longr X \times_S Y
$$
will be the product in the category.
\end{proof}

We will write this product as $X \hat{\times}_S Y$.

If $X$ is a formal scheme augmented over $S$, then the
morphism $q:X \to S$ is not schematic; however, it is ``formally
schematic'' in the sense that for all schemes $U \to S$, the
morphism
$$
U \cong U \times_S S \longr U \times_S X
$$
is formal; indeed, $\colim U \times_S X_n = U \times_S X$. Thus,
we can still define the push-forward functor on $\cO_X$-module
sheaves by
$$
(U \to S) \mapsto H^0(U \times_S X,\cF) \cong
\lim H^0(U \times_S X_n,i_n^\ast \cF).
$$
For the last isomorphism we use Lemma \ref{mod-formal}.

\begin{defn}\label{formal-affine}Let $X$ be a formal
scheme augmented over $S$. 
Let $\cI \subseteq \cO_X$ define
the closed inclusion $s:S \to X$; let $X_n \subseteq X$ be defined
by $\cI^n$. Define $X$ to be {\bf affine over $S$} if each
of the induced maps $X_n \to S$ is an affine morphism
of schemes.
\end{defn}

If $q:X \to S$ is affine, then $q_\ast (-)$ is an exact
functor. For we have a composition of total derived
functors
$$
Rq_\ast \cF \simeq \holim R(q_n)_\ast i_n^\ast \cF
$$
where $q_n:X_n \to S$ is the induced map. Since $q_n$ is
affine $(q_n)_\ast i_n^\ast \cF \simeq R(q_n)_\ast i_n^\ast \cF$;
thus we need to show that
$$
(q_n)_\ast i_n^\ast \cF \to (q_{n-1})_\ast i_{n-1}^\ast \cF
$$
is locally surjective. Since $(q_{n-1})_\ast = (q_n)_\ast j_\ast$
where $j:X_{n-1} \to X_n$ is the inclusion and since $(q_n)_\ast$
is exact (by Proposition \ref{qc-affine}), we need only show that
$$
i_n^\ast \cF \to j_\ast i_{n-1}^\ast \cF
$$
is locally surjective. Evaluated at $\Spec(A) \to X_n$, this is
exactly the morphism of sheaves obtained from the morphism
of presheaves 
$$
\cF(A) \longr \cF(A)/\cI(A)^{n-1}\cF(A).
$$

The exactness of $q_\ast$ has the following consequence.
The $\cO_S$-algebra $q_\ast \cO_X$ has an augmentation
to $\cO_S$ with augmentation ideal $q_\ast \cI$. Then
$$
q_\ast \cO_{X_n} =  q_\ast \cO_X/(q_\ast \cI)^n
$$
and 
$S \to X$ is formal and $q_\ast$ is a right adjoint
$$
q_\ast \cO_X \cong \lim q_\ast\cO_X/(q_\ast\cI)^n.
$$
The equivalence of categories between affine schemes over 
$S$ and quasi-coherent $\cO_S$-algebra sheaves now
specializes to the following result.

\begin{prop}\label{comp-affine}Consider the following two
categories:
\begin{enumerate}

\item the category of affine morphisms $q:X \to S$ with
section $s$ so that $s:S \to X$ is formal;

\item the category of augmented quasi-coherent $\cO_S$-algebra sheaves
$\cA$ so that $\cA$ is complete with respect to the augmentation 
ideal.
\end{enumerate}
Then the functor which assigns to $q:X \to S$ the algebra 
sheaf $q_\ast\cO_X$ with augmentation determined by $s:S \to X$
is an equivalence of categories.
\end{prop}

\subsection{Smoothness for formal schemes}

Here we spell out what it means for a formal scheme $X$
augmented over a base scheme $S$ to be smooth. 
There are many ways to define a smooth morphism of schemes.
We will focus on a definition using the sheaf of the differentials
and the cotangent sheaf as it generalizes well to the smooth setting.
In our applications, we will only need the case when $X \to S$ is a
separated morphism (see Definition \ref{affine-morphisms}). 
Note that any affine morphism is separated.

\begin{defn}\label{sheaf-of-diff} Let $X \to S$ be a separated morphism of
schemes, so that  diagonal
morphism $:\Delta:X \to X \times_S X$ is a closed embedding. 
Define the {\bf differentials} $\Omega_{X/S}$
on $X$ by
$$
\Omega_{X/S} = \Delta^\ast \cI/\cI^2
$$
where $\cI$ is the module of the closed embedding $\Delta$.

More generally, if factor that diagonal map as a closed embedding
followed by an open inclusion
$$
\xymatrix{
X \rto^j & V \rto & X \times_S X
}
$$
and set $\Omega_{X/S} = j^\ast \cI/\cI^2$ where $\cI$ is the
ideal defining $j$.
\end{defn}

If $X \to S$ is a morphism of schemes, the {\it cotangent complex}
$L_{X/S}$ is the total left derived functor of the differentials
functor $\Omega_{-/-}$ applied to morphism $X \to S$. As such,
it is a chain complex of quasi-coherent sheaves on $X$
{\it in the Zariski topology} and it comes with a natural augmentation
$L_{X/S} \to \Omega_{X/S}$.

Here's two conditions for smoothness. See \cite{Ill}, \S III.3.1.

\begin{prop}\label{reg-smooth} Let $q:X \to S$ be a flat 
and locally finitely presented morphism of schemes. Then $X$ is smooth over
$S$ if either of following two conditions is satisfied.
\begin{enumerate}

\item Any lifting problem
$$
\xymatrix{
Y_0 \rto \dto_{\subseteq} & X \dto^q\\
Y \rto \ar@{-->}[ur] & S
}
$$
where $Y_0 \to Y$ is a closed inclusion defined by a nilpotent
ideal has a solution;

\item The augmentation of the cotangent complex
$$
L_{X/S} \to \Omega_{X/S}
$$
is a quasi-isomorphism and the $\cO_X$-module $\Omega_{X/S}$ is locally free
of finite rank.
\end{enumerate}
\end{prop}

\begin{rem}\label{smooth-affine} If the morphism $q:X \to S$
is flat, locally finitely presented, and affine,  we can apply
Proposition \ref{qc-affine} to check the second condition of
Proposition \ref{reg-smooth}. Such a morphism $q:X \to S$
is smooth if and only if $q_\ast L_{X/S} \to q_\ast \Omega_{X/S}$
and $q_\ast \Omega_{X/S}$ is a locally-free module of finite
rank over $q_\ast \cO_X$.
\end{rem}

In order to pass to the formal setting, we spend a few paragraphs
on the sheaf of differentials and the cotangent complex.

Suppose we are given a morphism $q:X \to S$ of schemes with
a section $s$ and suppose that $s:S \to X$ is formal. Then
$s$ is a closed inclusion defined by an ideal-sheaf $\cI \subseteq \cO_X$.
Let $i_n: X_n \to X$ be the
closed subscheme defined by $\cI^n$.
Then we have the directed system of sheaves on $X$
\begin{equation}\label{tower-cotangent}
\cdots \to (i_n)_\ast \Omega_{X_n/S} \to (i_{n-1})_\ast \Omega_{X_{n-1}/S}
\to \cdots \to (i_1)_\ast \Omega_{X_1/S}
\end{equation}
and a morphism $\Omega_{X/S} \to \{(i_n)_\ast \Omega_{X_n/S}\}$ to this
directed system.

\begin{lem}\label{inverse-cotangent} For a formal scheme $X$
augmented over $S$, the natural map
$$
\Omega_{X/S} \to \lim \{(i_n)_\ast \Omega_{X_n/S}\}
$$ 
is an isomorphism.
\end{lem}

\begin{proof} There is an exact sequence of quasi-coherent
sheaves 
$$
(i_n)_\ast \cI^n/\cI^{2n} \to (i_n)_\ast i_n^\ast \Omega_{X/S}
\to (i_n)_\ast \Omega_{X_n/S} \to 0.
$$
The result follows from Lemma \ref{mod-formal}.
\end{proof}

The tower \ref{tower-cotangent} extends to a tower of chain complexes
\begin{equation}\label{tower-cotangent-complex}
\cdots \to (i_n)_\ast L_{X_n/S} \to (i_{n-1})_\ast L_{X_{n-1}/S}
\to \cdots \to (i_1)_\ast L_{X_1/S}.
\end{equation}
We use some concepts from  the homological algebra of towers
of chain complexes such as this.

\begin{defn}\label{pro-equivalence}Let $B$ be a commutative ring,
$J \subseteq B$ an ideal and $B_n = B/J^n$. Then there is a
tower of commutative rings
$$
\cdots \to B_n \to B_{n-1} \to \cdots \to B_1. 
$$
We consider the category 
$C_\ast\tow$ with objects the towers of chain complexes
$$
K = \{\cdots \to K_n \to K_{n-1} \to \cdots \to K_1\}
$$
with $K_n$ a bounded below chain complex of $B_n$
modules and each map $K_n \to K_{n-1}$ a morphism of
$B_n$-complexes -- so that the whole tower is a tower of $B$-complexes.
The morphisms in $C_\ast\tow$ are the evident
commutative ladders. We say that the tower $\{K_n\}$ is {\bf pro-trivial}
if for all $n$ there is a $k$ so that $K_{n+k} \to K_n$ is
chain homotopic to the zero map. We say that a morphism
$K \to L$ in $C_\ast\tow$ is a {\bf pro-equivalence} if the kernel
and cokernel are pro-trivial.

More generally, if $X$ is an $R$-functor and
$\cI \subseteq \cO_X$ is an ideal, we let $X_n \subseteq X$ be
the subscheme defined by $\cI^n$ and we have the category
$C_\ast\tow$ with objects
$$
K = \{\cdots \to (i_n)_\ast K_n \to (i_{n-1})_\ast K_{n-1} \to \cdots \to (i_1)_\ast K_1\}
$$
where each $K_n$ is a bounded below complex of quasi-coherent sheaves
on $X_n$. We say $K$ is pro-trivial if it is ``locally pro-trivial''; that is, if
for every Zariski  open $U \subseteq X$ and for all $n$ there is a $k$ so
that
$$
((i_{n+k})_\ast K_{n+k})(U) \to ((i_n)_\ast K_n)(U)
$$
is chain homotopic to zero. The definition of pro-equivalence follows as above.
\end{defn}

\begin{rem}\label{rems-on-pro} 1.) If $K \in C_\ast\tow$ has the property
that each $K_n$ is cofibrant $B_n$-complex (i.e., $K_n$ is level-wise
projective), then $K$ is pro-trivial if and only if for all $n$ there is
a $k$ so that $H_\ast K_{n+k} \to H_\ast K_n$ is the zero morphism.
The ``only if'' implication is clear. For the other, we may assume,
using a retraction argument, that $K_{n+k}$ is actually level-wise free
as a $B_n$-complex. Now use that $K_{n+k}$ is bounded below
and an induction argument to produce the chain homotopy. In the
scheme-theoretic setting let us assume that $X$ is quasi-compact.
Then we get a similar remark by requiring a complexes of locally free
quasi-coherent sheaves so
that for each Zariski open affine $U \subseteq Y$ and each $n$, there is a 
$k$ so that 
$$
H_\ast (\left.((i_{n+k})_\ast K_{n+k})\right\vert_U) \to
H_\ast (\left.((i_{n})_\ast K_n)\right\vert_U)
$$
is the zero morphism. 

2.) If $f:K \to L$ is a morphism in $C_\ast\tow$ with the property that
$f_n:K_n \to L_n$ is a surjective morphism between cofibrant
$B_n$-complexes. Then $\mathrm{Ker}(f_n)$ will also be cofibrant
as a $B_n$-complex; thus to check that $f$ is a pro-equivalence, we
need only check that for all $n$ there is a $k$ so that
$H_\ast \mathrm{Ker}(f_{n+k}) \to H_\ast \mathrm{Ker}(f_n)$
is the zero map. This remark also extends appropriately to schemes.

3.) Suppose $K \in C_\ast\tow$ is pro-trivial and has the property that
each $K_n$ is cofibrant as a $B_n$-complex. Then for all $n$ and all
$B_n$-modules $M$, there is a $k$ so that the map
$$
\mathrm{R}\Hom_{B_n}(K_n,M) \longr \mathrm{R}\Hom_{B_{n+k}}
(K_{n+k},M)
$$
is cochain homotopic to the zero map. Here $\mathrm{R}\Hom$ is
the total right derived functor of $\Hom$. Since $K_n$ is cofibrant,
there is a quasi-isomorphism of cochain complexes
$$
\mathrm{R}\Hom_{B_n}(K_n,M) \simeq \Hom_{B_n}(K_n,M).
$$
\end{rem}

We now give three different equivalent conditions which will be
the basis for smoothness in our formal setting.

First some notation.
Let $A$ be a commutative ring and $M$ an $A$-module. We let
$S_A(M) = \oplus_{s\geq 0} S_r(M)$ denote the symmetric algebra on $M$
where
$$
S_r(A) = (M \otimes_A \otimes_A\cdots\otimes_A M)/\Sigma_r
$$
is the $r$th symmetric power. Here $M$ appears $r$ times in the tensor
product. By convention, $S_0(M) = A$; hence
there is a natural $A$-algebra augmentation $S_A(M) \to A$. Let
$S_A(M)^\wedge$ denote the completion of $S_A(M)$ at the augmentation
ideal $I = \oplus_{s\geq 1} S_r(M)$.

\begin{prop}\label{smooth-conditions}
Let $B$ be a finitely generated $A$-algebra equipped with an
$A$-algebra augmentation $\epsilon:B \to A$. Let $J$ be the
kernel of $\epsilon$ and suppose that $B = \lim B/J^n$.
The the following statements are equivalent.
\begin{enumerate}

\item The $A$-module $J/J^2$ is finitely generated and
projective and any lifting problem
$$
\xymatrix{
A \rto \dto & C\dto\\
B \rto \ar@{-->}[ur] & C/I
}
$$
where $I$ is a nilpotent ideal and $C/I$ is annihilated by a power of $J$
has a solution where both triangles commute.

\item There is a projective $A$ module $P \subseteq J$ such that
induced map out of the completed symmetric algebra
$$
S_A(P)^\wedge \longr B
$$
is an isomorphism of $A$-algebras over $A$.

\item Let $B_n = B/J^n$. Then the natural map
$$
\{L_{B_n/A}\} \longr \{\Omega_{B_n/A}\}
$$
is a pro-equivalence of chain complexes, and $(\Omega_{B/A})^\wedge_J \cong
\lim \Omega_{B_n/A}$ is a finitely generated projective $B$-module.
\end{enumerate}
\end{prop}

\begin{exam}\label{affine-space} Let $R$ be a ring, $S = \Spec(R) = X$, 
$X = \Spec(R[[t_1,\cdots,t_n]])$, and $S \to X$ be defined
by the ideal $(t_1,\cdots,t_n)$. Then $S \to X$ is formal and one
easily checks directly that any of the three conditions of this
result are satisfied.
\end{exam}

\begin{proof} We begin with the implication that $(1) \Rightarrow (2)$.
We have that $B = A \oplus J$ as $A$-modules. Since $J \to J/J^2$
is surjective and the target is projective, we may choose an $A$-module
splitting. Write $P \subseteq J$ for the image of this splitting. This
gives the morphism $f:S_A(P)^\wedge \to B$ of (2). To show that is
an isomorphism, we filter source by the augmentation ideal $I$ and
the target by $J$. We will construct a morphism $g:B
\to S_A(P)^\wedge$ and show that $gf$ is the identity and that $fg$ induces
an isomorphism on the associated graded algebras. The implication will
follow.

We first note that by construction, the morphism
$$
S_A(P)^\wedge/I^2 \to B/J^2
$$
is an isomorphism. This constructs a map $B \to S_A(P)^\wedge/I^2$
so that the composite
\begin{equation}\label{projection}
S_A(P)^\wedge \to B \to S_A(P)^\wedge/I^2
\end{equation}
is the canonical projection.

Inductively, we contemplate the lifting problem
$$
\xymatrix{
A \rto\dto & S_A(P)/I^{n+1}\dto\\
B \rto \ar@{-->}[ur] & S_A(P)/I^{n}.
}
$$
It has a solution, by (1). Taking the limit gives a continuous morphism
of algebras $g:B \to S_A(P)^\wedge$ and the Equation \ref{projection}
implies that $gf:S_A(P)^\wedge \to S_A(P)^\wedge$ is the identity.
To show $fg$ is induces an isomorphism on the associated graded algebras,
we first examine the diagram on symmetric powers induced by $g$
$$
\xymatrix{
S_r(J/J^2) \rto^\cong \dto_m & S_r(I/I^2) \dto^\cong\\
J^r/J^{r+1} \rto &I^r/I^{r+1}
}
$$
where the vertical maps are induced by multiplication. The morphism
labeled $m$ is evidently surjection. Since the diagram commutes it
is an isomorphism. This shows that $g$ induces an isomorphism on the
associated graded algebras.

For the implication $(2) \Rightarrow (3)$ it sufficient to address the
case when  $P$ is free and finitely generated, as the general
case will be a retract of this one. Let $I \subseteq S_A(P)$ be
the augmentation and
$$
B_n = S_A(P)^\wedge/I^n \cong S_A(P)/I^n.
$$
Then a standard calculation -- using, for example,
Quillen's Fundamental Spectral Sequence of \cite{AQ} -- shows that
$H_pL_{B_n/A} = 0$ for $p > 1$ and
$$
H_pL_{B_n/A} \cong \brackets{B_n \otimes_A P}{p = 0}{I^n/I^{2n}}{p = 1.}
$$
Since $L_{B_n/A}$ is a cofibrant $B_n$-complex and 
$\Omega_{B_n/A}$ is a free $B_n$-module, the implication
follows from Remark \ref{rems-on-pro}.2.

We now work on the implication $(3) \Rightarrow (1)$. First note that
for every $A$-module $M$ there is a natural isomorphism
$$
\Der_A(B,A) \cong \Hom_A(J/J^2,M)
$$
or, put another way, that 
$$
(\Omega_{B/A})/J\cdot\Omega_{B/A} \cong A \otimes_B \Omega_{B/A}
\cong J/J^2.
$$
By Lemma \ref{inverse-cotangent} and Example \ref{qc-spf}, we have an isomorphism
$$
(\Omega_{B/A})^\wedge_J \cong \lim\Omega_{B_n/A}.
$$
Thus
$$
J/J^2 \cong (\Omega_{B/A})^\wedge/J\cdot\Omega_{B/A}^\wedge
$$
is a projective $A$-module. 

Now let us address the lifting problem. Since $C/I$ is annihilated by
a power of $J$, we can pass to the auxiliary lifting problem
$$
\xymatrix{
A \rto \dto & C\dto\\
B_n \rto \ar@{-->}[ur] & C/I
}
$$
This may not have a solution; however, by \cite{Ill}, Proposition III.2.2.4,
there is a natural obstruction to lifting in
$$
H^1\mathrm{R}\Hom_{B_n}(L_{B_n/A},I).
$$
We now apply Remark \ref{rems-on-pro}.3.
Since $\{L_{B_n/A}\} \to \{\Omega_{B_n/A}\}$ is a pro-equivalence,
there is an integer $k$ so that the induced morphism
$$
H^1\mathrm{R}\Hom_{B_n}(L_{B_n/A},I) \to
H^1\mathrm{R}\Hom_{B_m}(L_{B_{n+k}/A},I)
$$
is zero. Hence there is a solution to the larger lifting problem
$$
\xymatrix{
A \rto \dto & C\dto\\
B_{n+k} \rto \ar@{-->}[ur] & C/I
}
$$
and hence to the original lifting problem.
\end{proof}

In the following definition we will have a formal scheme $X$
augmented and affine over $S$. See Definition \ref{formal-affine}.

\begin{defn}\label{formal-smooth} Let $X$ be a formal
scheme augmented over $S$ and suppose the projection
morphism $q:X \to S$ is affine.

1.) The $X$ is {\bf formally finitely presented} over $S$ (or simply finitely
presented if the formal is understood) if for each Zariski open of $S$,
there are elements $x_1,\ldots,x_r$ of $q_\ast\cO_X(U)$ which generate
$(q_n)_\ast\cO_{Y_n}(U)$ as an $\cO_S(U)$ algebra for all $n$.

2.) The formal scheme $X$ {\bf smooth} over $S$ if
\begin{enumerate}

\item[a.)] $X \to A$ is flat and formally finitely presented type over $S$;

\item[b.)] $S$ has a cover by Zariski opens $U_i$ so that the morphism
of rings $\cO_S(U_i) \to q_\ast\cO_X(U_i)$ sastifies any of three
equivalent conditions of Proposition \ref{smooth-conditions}.
\end{enumerate}
\end{defn}

Of the three conditions of Proposition \ref{smooth-conditions}, the
one that globalizes well is the last. The second does not globalize
well in this generality because of the choices necessary to select
the projective module $P$; however, in the case of formal groups
we will see below {\bf where??} that the sheaf of invariant differntials
gives a natural and canonical choice for $P$. For now,
we record:

\begin{prop}\label{frml-cot-smooth}Let $X$ be a formal
scheme augmented over $S$ and suppose the projection
morphism $q:X \to S$ is affine.
Then $q:X \to S$ is smooth if and only if
\begin{enumerate}

\item $q: X \to A$ is flat and $X$ is formally finitely presented type over $S$;

\item the maps
$$
(i_n)_\ast L_{X_n/S} \longr (i_n)_\ast \Omega_{X_n/S}
$$
induce a pro-equivalence of towers; and

\item the module $q_\ast \Omega_{X/S} \cong \lim (q_n)_\ast
\Omega_{X_n/S}$ is locally free as a $q_\ast \cO_X$-module in
the Zariski topology. 
\end{enumerate}
\end{prop}

If $q_\ast \Omega_{X/S}$ is of constant rank $n$, we
say that $X \to S$ is smooth of {\it relative dimension $n$}. For
example, formal affine space (Example \ref{affine-space}) is
smooth of relative dimension $n$.

\subsection{Formal groups}

\begin{defn}\label{formal-group}Let $S$ be a scheme. A {\bf formal group}
$G$ over $S$ is a diagram
$$
\xymatrix{
G \ar@<.5ex>[r]^p & \ar@<.5ex>[l]^e S
}
$$
with $pe = 1_S$ so that the following conditions are satisfied:
\begin{enumerate}

\item The pair $e:S \to G$ is formal.

\item Let  $(G \times_S G)_{(e,e)}$ be the formal neighborhood of
$e \times e: S \to G \times_S G$. Then there is a product map
$$
\mu: (G \times_S G)_{(e,e)} \to G
$$
of formal schemes over $S$ and an inverse map $\chi: G \to G$ 
of formal schemes over $S$ so that $G$ becomes a group object
in the category of formal schemes over $S$.
\end{enumerate}
Write $\cO_G(e) \subseteq \cO_G$ for the ideal defining the
closed inclusion $e:S \to G$. This is the ideal of of functions vanishing
at the identity.

A {\bf homomorphism of formal groups} is a commutative diagram
$$
\xymatrix{
G\dto_f \ar@<.5ex>[r]^p & \ar@<.5ex>[l]^e S \dto^g\\
G' \ar@<.5ex>[r]^{p'} & \ar@<.5ex>[l]^{e'} S'\\
}
$$
which commute in the evident way with the multiplication maps and
inverse maps.
\end{defn}

Note that if we are given a homomorphism of formal groups
as in this definition, we can form the pull-back formal group 
$$
\xymatrix{
g^\ast G' \ar@<.5ex>[r]^p & \ar@<.5ex>[l]^e S
}
$$
over $S$, and then $f$ induces a homomorphism of formal groups
over $S$.

Note also that one can reformulate part (2) of Definition \ref{formal-group}
by stipulating a group structure on the functor $G(-)$.

We will not be interested in formal groups in general, but in ones
that are {\it affine} and {\it smooth} over $S$. 

\begin{exam}\label{fg-local}Let $S = \Spec(A)$ where $A$ is a commutative ring
ring and let $G$ be a smooth affine formal group of dimension $n$
over $S$. Since $G$ is affine and smooth, Propositions \ref{comp-affine}
and \ref{smooth-conditions}.2 imply that $G$ is the formal scheme
associated to completed algebra of the form $B = S_A(P)^\cmpl$ where
$P$ is a a projective A-module of rank $n$. Because
$G$ is a formal group, there is a continuous diagonal map
$$
\Delta: B \mathop{\longr} B \hat{\otimes}_A B
$$
and continuous antipodal map $\chi:B \to B$ such that $B$ becomes
a complete commutative Hopf algebra over $A$. (Here $\hat{\otimes}$
denotes the completed tensor product.) If $A$ is a local ring, the module
$P$ is free of rank $n$ and if we choose a basis
$x_1,\ldots,x_n$ of $P$ the diagonal map can be rewritten
$$
\Delta:A[[x_1,\ldots,x_n]] \longr A[[x_1,\ldots,x_n,y_1,\ldots,y_n]]
$$
and the power series in $2n$ variables
$$
F(x,y) = (F_1(x,y),\ldots,F_n(x,y)) \defeq
(\Delta(x_1),\ldots,\Delta(x_n))
$$
defines a {\it formal group law} of dimension $n$. Note that this formal
group law is commutative if $G$ is commutative. As a matter of notation,
it is often very convenient to write
$$
x +_F y = F(x,y).
$$
For example, let $g:G \to G'$ be a homomorphism of of smooth formal groups
over $\Spec(A)$. If $A$ is local and $G$ and $G'$ have dimensions $m$ and
$n$ respectively, then $g$ can be specified by a power series
$$
\phi(x) = (\phi_1(x),\ldots,\phi_n(x))
$$
in $m$-variables so that $\phi(x+_F y) = \phi(x) +_{F'} \phi(y)$.
\end{exam}

We now introduce the moduli stack $\cM_\fg$ of affine smooth
commutative formal groups of dimension 1. Although we call this object a stack
right from the start, we will have to prove that it is indeed an algebraic
stack. See Theorem \ref{fg-algebraic} below.

\begin{defn}\label{stack-of-fgs}Let $\Aff/\ZZ$ be the category
of affine schemes over $\Spec(\ZZ)$.\footnote{This category is, of course, 
the opposite category of the category of commutative rings.}
We define a category
$\cM_\fg$ fibered in groupoids over $\Aff/\ZZ$ as follows.
The objects of $\cM_\fg$ consist of affine smooth {\it 
commutative} formal groups
of dimension $1$ 
$$
\xymatrix{
G \ar@<.5ex>[r]^p & \ar@<.5ex>[l]^e S 
}
$$
where $S \in \Aff/\ZZ$. A morphism in $\cM_\fg$ is a homomorphism
of formal groups
$$
\xymatrix{
G\dto_f \ar@<.5ex>[r]^p & \ar@<.5ex>[l]^e S \dto^g\\
G' \ar@<.5ex>[r]^{p'} & \ar@<.5ex>[l]^{e'} S'\\
}
$$
so that the induced homomorphism $G \to g^\ast G'$ is an 
{\bf isomorphism} of formal groups over $S$. 

The augmentation $\cM_\fg \to \Aff/\ZZ$ sends $G \to S$
to $S$.
\end{defn}

If $S \in \Aff/\ZZ$, let us define $\cM_\fg(S)$ to the groupoid
of formal groups (affine, smooth, commutative, and of dimension 1)
over $S$. Thus the morphisms of $\cM_\fg(S)$ are isomorphism
of formal groups over $S$. Let us write
$$
\Hom_{\cM_\fg(S)}(G,H)\defeq \Iso_S(G,H).
$$

We now begin the process of showing that $\cM_\fg$ is an algebraic
stack. The notion of a {\it stack} is defined in Definition 3.1
of \cite{Laumon}. 

\begin{lem}\label{fflat-proj}Let $X$ be a quasi-compact and quasi-seperated scheme
and $\cF$ is a finitely generated locally free sheaf of rank 1 on $X$. Then there
is a finite set of Zariski open subschemes $U_i \subseteq X$
so that if $Y =\sqcup\ U_i$ and if $f:Y \to X$ is the
evident map, then $f^\ast \cM \cong \cO_Y$. In particular,
$f:Y \to X$ is locally of finite presentation and $Y$ is quasi-compact
and quasi-separated.
\end{lem}

\begin{proof} Under the hypotheses on $X$ there
is a morphism $f:X \to P^n$ for some $n$ so that $f^\ast\cO(1) \cong \cF$.
Let $U_i \to S$ be the pull-back of the 
standard affine $i:\AA^n \to P^n$.
\end{proof}

\begin{lem}\label{prestack}The category $\cM_\fg$ fibered in
groupoids over $\Aff/\ZZ$ is a stack in the fpqc topology.
\end{lem}

\begin{proof}First, we must prove that isomorphisms of
formal groups form a sheaf in the following sense.
Let $S \in \Aff/\ZZ$ and $G$ and $H$ two formal groups
over $S$. Suppose $f:T \to S$ is faithfully flat. Then
we need to show that if $\phi:d^\ast G \to d^\ast H$
is an isomorphism of formal groups over $T$ so that
we have a commutative diagram of formal groups over
$T \times_S T$
$$
\xymatrix{
d_1^\ast d^\ast G \rto^{d_1^\ast \phi} \dto_\cong &
d_1^\ast d^\ast H \dto^\cong\\
d_0^\ast d^\ast G \rto_{d_0^\ast \phi}& d_0^\ast d^\ast H
}
$$
then there is a unique isomorphism $\phi:G \to H$ over $S$ so that
$f^\ast \psi = \phi$. But this follows because faithfully flat descent is
an equivalence of categories. See Remark \ref{ff-descent}
and Proposition \ref{comp-affine}.

Second, we must prove that we have effective descent for formal
groups. Again we have a faithfully flat morphism $f:T \to S$ and
a affine smooth commutative 1-dimensional formal group $H$
over $T$ equipped with an isomorphism of formal groups
$$
\phi:d_1^\ast H \longr d_0^\ast H
$$
over $T \times_S T$ which satisfies the evident coycle condition.
By faithfully flat descent -- Remark \ref{ff-descent} and Proposition
\ref{comp-affine} again -- there
is an affine formal group $G$ over $S$ so that $f^\ast G \cong H$; that is,
there is a cartesian diagram 
\begin{equation}\label{effective-diag}
\xymatrix{
H \rto^{F}\dto_p & G \dto^q\\
T \rto_F & S.
}
\end{equation}
We must show that $G$ is smooth and 1-dimensional. It is certainly
flat and formally of finite type over $S$, again by faithfully flat
descent and Lemma \ref{fflat-inherits}. 
Write $p_n:H_n \to T$ and $q_n:G_n \to S$ for the restrictions of
$p$ and $q$ to the infinitesimal neighborhoods and write
$j_n:H_n \to H$ and $i_n:G_n \to G$ for the inclusions. Then we must show that 
$$
(i_n)_\ast L_{G_n/S} \longr (i_n)_\ast \Omega_{G_n/S}
$$
is a pro-equivalence. Since $F:T \to S$ is faithfully flat, and $S$
and $T$ are affine, Remark \ref{rems-on-pro}.1 implies that it is sufficient
to show
$$
F^\ast(i_n)_\ast L_{G_n/S} \longr
F^\ast(i_n)_\ast \Omega_{G_n/S}
$$
is a pro-equivalence. Since we have a cartesian square
$$
\xymatrix{
H_n \rto^{F_n} \dto_{j_n} & G_n \dto^{i_n}\\
H \rto_{F} & G
}
$$
we have $F^\ast (i_n)_\ast = (j_n)_\ast F_n^\ast$ and we need only show
$$
(j_n)_\ast F_n^\ast L_{G_n/S} \longr
(j_n)_\ast F_n^\ast \Omega_{G_n/S}
$$
is a pro-equivalence.
Since Equation \ref{effective-diag} is a pull-back
and $f$ is flat, flat base change for the cotangent complex implies
this last set of morphisms is equivalent to
$$
(j_n)_\ast L_{H_n/T} \longr (j_n)_\ast \Omega_{H_n/T}
$$
which is a pro-equivalence by assumption.

It remains to
show that $q_\ast \Omega_{G/S} = \lim (q_n)_\ast \Omega_{G_n/S}$ is a rank 1
projective as an $q_\ast \cO_{G}$-module. Since diagram \ref{effective-diag}
is cartesian, we we have
$$
f^\ast q_\ast \Omega_{G/S} = p_\ast F^\ast \Omega_{G/S} \cong
p_\ast \Omega_{H/T}.
$$
Thus we can apply Lemma \ref{fflat-inherits}.3.
\end{proof}

